OptiSeq: Ordering Examples On-The-Fly for In-Context Learning

Developers using LLMs and LLM-based agents in their applications have provided plenty of anecdotal evidence that in-context-learning (ICL) is fragile. In this paper, we show that in addition to the quantity and quality of examples, the order in which the in-context examples are listed in the prompt affects the output of the LLM and, consequently, their performance. While prior work has explored improving ICL through dataset-dependent techniques, we introduce OptiSeq, a purely inference-time, dataset-free optimization method that efficiently determines the best example order. OptiSeq leverages log probabilities of LLM-generated outputs to systematically prune the search space of possible orderings and recommend the best order(s) by distinguishing orderings that yield high levels of accuracy and those that underperform. Extensive empirical evaluation on multiple LLMs, datasets, and prompts demonstrate that OptiSeq improves accuracy by 5.5 - 10.5 percentage points across multiple tasks.

==> commented_out.tex <==
\section{\ours}

Given a set of in-context examples $E = \{e_1, ..., e_n\}$ and a language model $M$, we aim to find the optimal ordering $\pi^*$ of examples that maximizes the model's performance on target tasks. Each example $e_i$ consists of an input-output pair $(x_i, y_i)$.
Let $\Pi(E)$ be the set of all possible permutations of the in-context examples $E$. For a set of $n$ examples, $|\Pi(E)| = n!$. Let $Q$ be the Natural Language input. 
For each permutation $\pi_j \in \Pi(E)$:

\begin{enumerate}
    \item Construct prompt $P_j$ by concatenating examples in order $\pi_j$:
    \begin{equation}
        P_j = \text{concat}(\pi_j(e_1, ..., e_n))
    \end{equation}

    \item Generate outputs using the language model:
    \begin{equation}
        Y_j = M(P_j)
    \end{equation}
    where $Y_j$ represents the set of generations for permutation $j$
\end{enumerate}

\subsection{Evaluation Phase}
For each permutation $\pi_j$:

\begin{enumerate}
    \item Construct a modified prompt $P'$ without in-context examples
    \item For each generation $y_{j,k} \in Y_j$:
    \begin{itemize}
        \item Append generation to modified prompt: $P'_k = \text{concat}(P', y_{j,k})$
        \item Calculate log probabilities of input tokens:
        \begin{equation}
            \text{score}(y_{j,k}) = \sum_{t=1}^{|x_k|} \log P(x_{k,t}|P'_k)
        \end{equation}
        where $x_{k,t}$ represents the $t$-th token of the input corresponding to generation $k$
    \end{itemize}

    \item Calculate total score for permutation $\pi_j$:
    \begin{equation}
        S(\pi_j) = \sum_{k=1}^{|Y_j|} \text{score}(y_{j,k})
    \end{equation}
\end{enumerate}

Select the optimal permutation:
\begin{equation}
    \pi^* = argmax_{\pi_j \in \Pi(E)} S(\pi_j)
\end{equation}

\begin{algorithm}
\caption{\ours}
\begin{algorithmic}[1]
\Require Set of examples $E$, Language model $M$
\Ensure Optimal permutation $\pi^*$
\State Initialize $\text{best\_score} = -\infty$, $\pi^* = \text{null}$
\State $\Pi(E) \gets \text{GeneratePermutations}(E)$
\For{each $\pi_j$ in $\Pi(E)$}
    \State $P_j \gets \text{ConstructPrompt}(\pi_j)$
    \State $Y_j \gets \text{GenerateOutputs}(M, P_j)$
    \State $P' \gets \text{ConstructBasePrompt}()$
    \State score $\gets 0$
    \For{each $y$ in $Y_j$}
        \State $P'_k \gets \text{Concatenate}(P', y)$
        \State score $\gets$ score $+$ CalculateLogProbabilities$(M, P'_k)$
    \EndFor
    \If{score $>$ best\_score}
        \State best\_score $\gets$ score
        \State $\pi^* \gets \pi_j$
    \EndIf
\EndFor
\State \Return $\pi^*$
\end{algorithmic}
\end{algorithm}




\subsection{Complexity Analysis}
\begin{itemize}
    \item \textbf{Time Complexity}: $O(n! \cdot m)$ where $n$ is the number of examples and $m$ is the average length of inputs
    \item \textbf{Space Complexity}: $O(n!)$ for storing permutations and their scores
\end{itemize}



\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{latex/figures/optiseq_diagram.pdf}
    \caption{\ours methodology}
    \label{fig:optiseq:method}
\end{figure*}

\section{Methodology}
Our approach, \textbf{\ours}, is designed to address the sensitivity of large language models (LLMs) to the ordering of in-context examples in ICL. \ours systematically evaluates all possible orderings of in-context examples and selects the one that maximizes prediction accuracy. The methodology consists of four key steps:

\begin{enumerate}
    \item \textbf{Generate Sequences for All Possible Orders}: Given $n$ in-context examples, there are $n!$ possible permutations of those examples. In this step, we generate sequences for all these orderings to comprehensively explore how different arrangements affect model predictions. The intuition behind this step is to treat each ordering as a potential hypothesis, allowing the model to evaluate which order leads to the most coherent prediction for the test utterance. 

    \item \textbf{Remove In-Context Examples from the Prompt}: After generating sequences, we remove the in-context examples from the prompt, isolating the model’s prediction. This step ensures that the test utterance and predicted sequence are not biased by the presence of examples in the prompt, allowing us to evaluate the sequence purely on its merits. The rationale is to strip the task to its essence—how well the model generalizes the test utterance based on prior examples, rather than relying on any specific example being present during inference.

    \item \textbf{Generate Log Probabilities for Each Sequence}: For each generated sequence, the model calculates the log probabilities of tokens in the sequence. This allows us to quantify the confidence of the model in each prediction. The intuition here is that sequences with higher log probabilities are more likely to be correct, as the model has more confidence in its token-level predictions. This step captures the likelihood of each possible sequence under different in-context orderings.

    \item \textbf{Select the Sequence with the Maximum Confidence Score}: Finally, we select the sequence that corresponds to the highest overall confidence score, as determined by the log probabilities. This step leverages the model’s internal scoring mechanism to pick the most reliable sequence. The intuition is simple: the higher the confidence in a sequence, the more likely it is that the model has accurately understood the test utterance in relation to the examples provided.
\end{enumerate}

By following these steps, \textbf{\ours} not only improves the model’s ability to generate accurate API sequences but also mitigates the problem of ordering sensitivity, which often leads to significant performance fluctuations across different prompts.

\subsection{Intuition Behind Each Step}

\begin{itemize}
    \item \textbf{Generating all possible sequences}: This brute-force approach explores all configurations of in-context examples to avoid missing an optimal order, acknowledging that each permutation may provide the model with different contextual signals.

    \item \textbf{Removing in-context examples from the prompt}: This focuses the model purely on the new utterance and sequence prediction, eliminating any undue influence that the specific examples might have when they remain in the prompt during prediction.

    \item \textbf{Generating log probabilities}: The use of log probabilities as a measure of confidence is crucial. It provides an objective, model-internal metric for evaluating how well the model believes it has understood and predicted the correct sequence, enabling a quantitative comparison of different orders.

    \item \textbf{Selecting the sequence with maximum confidence}: This final step aligns the prediction with the model’s highest level of certainty, ensuring that we choose the sequence that the model internally rates as the most accurate.
\end{itemize}

Through this methodology, \textbf{\ours} systematically reduces the uncertainty introduced by example ordering and helps identify the optimal sequence, enhancing performance in tasks that rely on accurate API sequence generation.



\begin{itemize}
    \item 3 examples in the right order compared to more examples (5) in random order. Latency + accuracy. IBM-20b on tool bench : 4 shot - 55.80 \% and 5 shot - 57.02 \% \ours : 62.93 \%. Mistral 4 shot on tool bench- 43.36, 5 shot - 43.78, \ours - 48.26. ibm-20b on restgpt 4 shot 38.21 \%, 5 shot: 41.22 \ours: 46.49 \%. Mistral on restgpt 4-shot: 47.70, 5 shot: 50.95 \% \ours: 55.41
    \item Latency experiments (batched inference).
    \item OOD experiment. OOD examples in the right order vs random order in-distribution examples. OOD : meta\_8b tool bench \ours : 47.86 \% , mistral\_7\_8b tool bench \ours: 46.84 \% , restgpt: meta\_8b: 50.31 \% mistral\_7\_8b: 49.08 \%
    \item precision and recall
    
\end{itemize}

\begin{comment}
  \begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{latex/plots/compare_4_5_shot_tool_rest_opti.pdf}
    \caption{Comparing 3,4 and 5 shot random selection strategy with 3 shot \ours (in red) \textbf{Add TopK}.}
    \label{fig:enter-label}
\end{figure}  

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{latex/plots/OOD_experiment.pdf}
    \caption{Comparing In-distribution (ID) with Out-of-distribution performance (OOD). Here ToolBench uses in-context examples from RestGPT and vice-versa \textbf{Add TopK}}
    \label{fig:enter-label}
\end{figure}
\end{comment}



\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.2} % Increase row height
\setlength{\tabcolsep}{5pt} % Increase column spacing
\small
\begin{tabular}{c|l|cccc|c}
\hline
\textbf{Dataset} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}Random \\ Selection\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TopK \\ Selection\end{tabular}} & \textbf{\ours} & \textbf{\begin{tabular}[c]{@{}c@{}}TopK++\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Improvement \\ (\ours - TopK)\end{tabular}} \\ \hline
Tool Bench & llama-3-8b-instruct & 71.47 / 70.58 & 71.63 / 70.45 & 77.75 / 77.12 & 75.77 / 74.58 & 6.12 / 6.67 \\
 & llama-3-70b-instruct & 82.57 / 82.08 & 83.04 / 82.95 & 85.03 / 84.07 & 84.79 / 83.88 & 1.99 / 1.12 \\
 & granite-20b-code-instruct & 75.83 / 75.18 & 77.35 / 77.10 & 81.78 / 81.64 & 80.72 / 79.34 & 4.43 / 4.54 \\
 & granite-13b-instruct-v2 & 72.03 / 74.85 & 73.20 / 76.29 & 76.55 / 78.58 & 75.16 / 77.04 & 3.35 / 2.29 \\
 & mixtral-8x7b-instruct-v01 & 74.16 / 76.15 & 73.78 / 76.33 & 81.85 / 84.21 & 80.12 / 81.97 & 8.07 / 7.88 \\ \hline
RestGPT & llama-3-8b-instruct & 75.43 / 75.04 & 75.74 / 75.62 & 78.69 / 78.72 & 77.52 / 77.11 & 2.95 / 3.10 \\
 & llama-3-70b-instruct & 74.70 / 75.35 & 74.22 / 75.15 & 77.64 / 78.07 & 76.79 / 77.13 & 3.42 / 2.92 \\
 & granite-20b-code-instruct & 74.76 / 74.23 & 75.28 / 74.84 & 76.27 / 75.01 & 75.86 / 74.79 & 0.99 / 0.17 \\
 & granite-13b-instruct-v2 & 74.12 / 74.56 & 74.68 / 75.12 & 76.23 / 76.78 & 75.89 / 76.34 & 1.55 / 1.66 \\
 & mixtral-8x7b-instruct-v01 & 74.56 / 74.84 & 75.24 / 75.76 & 77.53 / 77.47 & 77.10 / 77.32 & 2.29 / 1.71 \\ \hline
\end{tabular}
\caption{Precision/Recall in \% and Improvement of \ours over TopK}
\end{table*}


\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} % Increase row height
\setlength{\tabcolsep}{2.5pt} % Increase column spacing
%\small
\begin{tabular}{c|l|cc|cc|cc|cc|cc}
\hline
\textbf{Dataset} & \multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Random}} & \multicolumn{2}{c|}{\textbf{Top-K}} & \multicolumn{2}{c|}{\textbf{\ours}} & \multicolumn{2}{c|}{\textbf{Top-K++}} & \multicolumn{2}{c}{\textbf{Improve.}} \\
 &  & \textbf{Prec.} & \textbf{Rec.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{Prec.} & \textbf{Rec.} \\ \hline
Tool Bench & llama-3-8b-instruct & 71.47 & 70.58 & 71.63 & 70.45 & \textbf{77.75} & \textbf{77.12} & \underline{75.77} & \underline{74.58} & 6.12 & 6.67 \\
 & llama-3-70b-instruct & 82.57 & 82.08 & 83.04 & 82.95 & \textbf{85.03} & \textbf{84.07} & \underline{84.79} & \underline{83.88} & 1.99 & 1.12 \\
 & granite-20b-code-instruct & 75.83 & 75.18 & 77.35 & 77.10 & \textbf{81.78} & \textbf{81.64} & \underline{80.72} & \underline{79.34} & 4.43 & 4.54 \\
 & granite-13b-instruct-v2 & 72.03 & 74.85 & 73.20 & 76.29 & \textbf{76.55} & \textbf{78.58} & \underline{75.16} & \underline{77.04} & 3.35 & 2.29 \\
 & mixtral-8x7b-instruct-v01 & 74.16 & 76.15 & 73.78 & 76.33 & \textbf{81.85} & \textbf{84.21} & \underline{80.12} & \underline{81.97} & 8.07 & 7.88 \\ \hline
RestGPT & llama-3-8b-instruct & 75.43 & 75.04 & 75.74 & 75.62 & \textbf{78.69} & \textbf{78.72} & \underline{77.52} & \underline{77.11} & 2.95 & 3.10 \\
 & llama-3-70b-instruct & 74.70 & 75.35 & 74.22 & 75.15 & \textbf{77.64} & \textbf{78.07} & \underline{76.79} & \underline{77.13} & 3.42 & 2.92 \\
 & granite-20b-code-instruct & 74.76 & 74.23 & 75.28 & 74.84 & \textbf{76.27} & \textbf{75.01} & \underline{75.86} & \underline{74.79} & 0.99 & 0.17 \\
 & granite-13b-instruct-v2 & 74.12 & 74.56 & 74.68 & 75.12 & \textbf{76.23} & \textbf{76.78} & \underline{75.89} & \underline{76.34} & 1.55 & 1.66 \\
 & mixtral-8x7b-instruct-v01 & 74.56 & 74.84 & 75.24 & 75.76 & \textbf{77.53} & \textbf{77.47} & \underline{77.10} & \underline{77.32} & 2.29 & 1.71 \\ \hline
\end{tabular}
\caption{Precision(Prec.) and Recall(Rec.) in \% and Improvement of \ours over Top-K}
\label{table:prec:rec}
\end{table*}


%While LLMs exhibit promising capabilities, there remains a noticeable gap in understanding the nuances of in-context example ordering and its effect on model performance. This study addresses this gap by systematically analyzing how different orderings of in-context examples impact the accuracy of API sequence generation. Rather than focusing on broad prompt design, we delve specifically into the challenge of optimizing in-context example ordering.

%To tackle this issue, we introduce \ours, a novel approach for selecting the optimal order of in-context examples. \ours works by generating all possible orderings of the examples, computing the log probabilities for each generated sequence, and selecting the sequence with the highest confidence score. This method significantly improves prediction accuracy, outperforming both random selection and state-of-the-art approaches. Furthermore, we propose Efficient \ours, a variant that reduces the number of LLM calls, maintaining robust performance while optimizing resource use.

%Through a series of experiments, we demonstrate that the ordering of in-context examples plays a pivotal role in determining the accuracy of API sequence prediction. By identifying optimal configurations for in-context example ordering, our research enhances the reliability and efficiency of LLM-based tool prediction systems. Future work will explore further reductions in LLM calls and refine the methodology to handle ambiguous or edge-case utterances more effectively


\begin{table*}[ht]
    \centering
    \small
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{p{3.5cm} p{5.5cm} c c c c}
\toprule
\textbf{Utterance} & \textbf{Generated Sequence} & \textbf{Precision} & \textbf{Recall} & \textbf{Accuracy} & \textbf{Log Prob} \\
\midrule
\multirow{6}{*}{\parbox{3.5cm}{\tiny I need to retrieve the pending messages from my device with ID 123456. Please provide the pending messages using my TrumpetBox Cloud API KEY.}} 
& \tiny \textcolor{blue}{\texttt{trumpetbox\_cloud.devices\_getasingledeviceinfofromaccount, trumpetbox\_cloud.messages\_getpendingmessagesfromaccount}} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{-1.54} \\
& \tiny \texttt{trumpetbox\_cloud.messages\_getpendingmessagesfromaccount} & \textbf{100.0} & 50.0 & 0.0 & -3.54 \\
& \tiny \textcolor{blue}{\texttt{trumpetbox\_cloud.devices\_getasingledeviceinfofromaccount, trumpetbox\_cloud.messages\_getpendingmessagesfromaccount}} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{-1.54} \\
& \tiny \texttt{trumpetbox\_cloud.messages\_getpendingmessagesfromaccount} & \textbf{100.0} & 50.0 & 0.0 & -3.54 \\
& \tiny \texttt{trumpetbox\_cloud.messages\_getpendingmessagesfromaccount} & \textbf{100.0} & 50.0 & 0.0 & -3.54 \\
& \tiny \textcolor{blue}{\texttt{trumpetbox\_cloud.devices\_getasingledeviceinfofromaccount, trumpetbox\_cloud.messages\_getpendingmessagesfromaccount}} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{-1.54} \\
\midrule
\multirow{6}{*}{\parbox{3.5cm}{\tiny I need to track the performance of my family's crypto investments. Can you provide me with a list of our current positions for Bitcoin, Ethereum, and Ripple, along with their historical data and market trends?}} 
& \tiny \textcolor{blue}{\texttt{crypto\_grana.list.position.for.each.crypto, crypto\_grana.list.histories}} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{-1.66} \\
& \tiny \texttt{crypto\_grana.list.position.for.each.crypto} & \textbf{100.0} & 50.0 & 0.0 & -5.61 \\
& \tiny \texttt{crypto\_grana.list.position.for.each.crypto} & \textbf{100.0} & 50.0 & 0.0 & -5.61 \\
& \tiny \textcolor{blue}{\texttt{crypto\_grana.list.position.for.each.crypto, crypto\_grana.list.histories}} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{-1.66} \\
& \tiny \texttt{crypto\_grana.list.position.for.each.crypto} & \textbf{100.0} & 50.0 & 0.0 & -5.61 \\
& \tiny \textcolor{blue}{\texttt{crypto\_grana.list.position.for.each.crypto, crypto\_grana.list.histories}} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{-1.66} \\
\bottomrule
\end{tabular}%

    }
    \caption{Generated Sequences and Metrics for Different Utterances}
\end{table*}

